Tetraquarks composed of 4 heavy quarks

In the current work spectroscopy and possibility of observation at the LHC of tetraquarks composed of 4 heavy quarks is discussed. Tetraquarks concerned are T_{4c}=[cc][cc]$, T_{4b}=[bb][bb] and T_{2[bc]}=[bc][bc]. By solving nonrelativistic Schroedinger equation masses of these states are found with the hyperfine splitting accounted for. It is shown that masses of tensor tetraquarks T_{4c}(2++) and T_{2[bc]}(2++) are high enough to observe these states as peaks in the invariant mass distributions of heavy quarkonia pairs in pp -> T_{4c}+X -> 2J/\psi+X, pp -> T_{2[bc]}+X -> 2B_{c}+X and pp -> T_{2[bc]}+X -> J/\psi\Upsilon(1S)+X channels while T_{4b} is under the threshold of decay into a vector bottomonia pair.

==> masses.tex <==
% (* cc *)
\newcommand{\mDiqCC}{3.13}
\newcommand{\RDiqCC}{0.523}
\newcommand{\RMesonCC}{0.75}
\newcommand{\kappaDiqCC}{12.8}
\newcommand{\kappaMesonCC}{42.8}
\newcommand{\MtetraCC}{6.124}
\newcommand{\MScalarCC}{5.966}
\newcommand{\DMScalarCC}{-228.}
\newcommand{\MAxialCC}{6.051}
\newcommand{\DMAxialCC}{-142.}
\newcommand{\MTensorCC}{6.223}
\newcommand{\DMTensorCC}{29.5}

% ( * bb *)
\newcommand{\mDiqBB}{9.72}
\newcommand{\RDiqBB}{1.35}
\newcommand{\RMesonBB}{2.27}
\newcommand{\kappaDiqBB}{5.52}
\newcommand{\kappaMesonBB}{27.1}
\newcommand{\MtetraBB}{18.857}
\newcommand{\MScalarBB}{18.754}
\newcommand{\DMScalarBB}{-544.}
\newcommand{\MAxialBB}{18.808}
\newcommand{\DMAxialBB}{-490.}
\newcommand{\MTensorBB}{18.916}
\newcommand{\DMTensorBB}{-382.}

 %(* bc *)
\newcommand{\mDiqBC}{6.45}
\newcommand{\RDiqBC}{0.722}
\newcommand{\RMesonBC}{1.29}
\newcommand{\kappaDiqBC}{6.43}
\newcommand{\kappaMesonBC}{27.1}
\newcommand{\MtetraBC}{12.491}
\newcommand{\MScalarBCa}{12.359}
\newcommand{\DMScalarBCa}{-191.}
\newcommand{\MScalarBCb}{12.471}
\newcommand{\DMScalarBCb}{-78.7}
\newcommand{\MAxialBCa}{12.424}
\newcommand{\DMAxialBCa}{-126.}
\newcommand{\MAxialBCb}{12.488}
\newcommand{\DMAxialBCb}{-62.5}
\newcommand{\MAxialBCc}{12.485}
\newcommand{\DMAxialBCc}{-64.9}
\newcommand{\MTensorBC}{12.566}
\newcommand{\DMTensorBC}{16.1}

